An Assessment of Contamination in the thermal-SZ Map Using Cross Correlations

We search for the potential contamination in the Planck thermal Sunyaev-Zeldovich (tSZ) map by calculating the cross-correlation between the tSZ signal and weak lensing by large scale structure and the Cosmic Microwave Background (CMB). The lensing data we use is the convergence map from the Red Sequence Cluster Lensing Survey (RCSLens) and the Planck CMB lensing map. We reconstruct the tSZ $y$ map with a Needlet Internal Linear Combination method using the HFI sky maps from the Planck satellite. We remove the CMB signal while minimizing the residual noise. The cross correlation signal from our reconstructed $y$ map is consistent with that from the Planck team's NILC $y$ map. The CIB and galactic dust emission are two potential sources of contamination in the reconstructed $y$ map. We remove the CIB signal by subtracting the CIB maps reconstructed by Planck collaboration from the raw temperature maps. We find that cross-correlation between the CIB and galactic lensing contributes to $(7.5\pm6.0)\%$ in the Planck NILC tSZ cross galactic lensing signal within $100<\ell<2000$, which implies that previous detections of the tSZ cross galactic lensing is robust to CIB contaminations. In contrast, the Planck NILC tSZ cross CMB lensing is biased by $(18.4\pm2.8)\%$ in the same $\ell$ range. Galactic dust contamination is tested by projecting out a grey-body dust models with different dust spectral indices. Galactic dust does not affect galactic lensing cross tSZ signal significantly.

==> report.tex <==
Cover Letter

Dear Referee:

Thank you for your kind comments. Some of them are really helpful to improve our manuscript. Before replying to each of the comments specifically, we would like to summarize the most important modification to the results of the revised manuscript.

The level and error of CIB contaminations changes a little bit because we use the new method to calculate the error (as you kindly suggested) of cross-correlation. Besides, we adopt the tSZ-projected out CMB lensing map from the newest Planck 2018 data release. We delete the discussion in Appendix C of the old manuscript because it does not apply to the new CMB lensing map. We add a new Appendix C to discuss whether the tSZ residual in the CMB lensing map affects the \phi x y signal.

Here are the reply to your comments: 

Abstract:
- It is misleading to not mention that in the measurement of the tSZ - CMB lensing cross-correlation signal, a CIB bias of the magnitude given here was indeed subtracted. As currently written, the abstract implies that the measurement did not correct for this bias, which is not true.

We add a sentence indicating that we use the CIB subtracted y map for both galactic and CMB lensing to calculate lensing-y cross-correlation.

- The Planck CIB maps will have some level of tSZ contamination in them, and thus cannot be treated simply as CIB-only maps.

We discuss it in the last paragraph of Section 4.1. 

Introduction:
- The abundance of galaxy clusters depends much more strongly on sigma_8 than Omega_m. This statement should be corrected.

Corrected in the revised version.

- MILCA stands for "modified internal linear combination algorithm"; this should be corrected.

Corrected in the revised version.

- The X-ray hydrostatic equilibrium (HSE) mass bias problem may have nothing to do with the missing baryons problem in low-mass halos. For example, the HSE bias can be sourced by non-thermal pressure support due to turbulence in the ICM, which has nothing to do with the missing baryons problem in 10^12 or 10^13 M_sun halos.

Corrected in the revised version. We specify the situation to be only high-mass halos.

- The tSZ-lensing cross-correlation detection in van Waerbeke et al. (2014) was 6 sigma (quoting directly from the abstract of their paper), not 7 sigma as stated here.

Corrected in the revised version. 

- The CIB is not "redshifted starlight" as stated here. It is redshifted thermal emission from dust grains heated by starlight.

Corrected in the revised version. 

Formalism:
- Why is this formalism introduced if no physical models are ever fit to the signals? I can see that the frequency dependence of the components must be described, but no models for the gas or CIB are fit to the data, as far as I can tell. Thus, most of this section seems unnecessary.

This section serves as background information of the cross-correlation. It indicates why people do cross-correlations and why it is important to test the robustness of previous results.

- Why is a halo model implicitly introduced for the CIB (i.e., the use of L_500), but perturbation theory is used for the other fields? Again, I do not see the necessity of introducing most of the modeling here.

This model is used for extrapolating to get 100-217GHz CIB maps.

Data and Method:
- Why is the Planck LFI data not used in this analysis?
- Does the consistency of the results shown here with those derived from the Planck y-map imply that the LFI data is irrelevant?

We did not use LFI data partly because Planck only uses LFI at l<300 which is below the angular scale that we are concerning about. Also the dust and CIB signal at LFI channels are quite low. 

- The Planck CIB maps will have non-zero tSZ residuals. How is this treated in the analysis?

We discuss it in the last paragraph of Section 4.1.

- One issue the authors may want to address, or at least mention, is the tSZ cluster mask applied to the 2015 Planck CMB lensing map, which obviously affects the tSZ - CMB lensing cross-correlation in a non-trivial way.
- Similarly, what about tSZ signal that has leaked into the CMB lensing map, which could contaminate the tSZ - CMB lensing cross-correlation?

We have changed the CMB lensing map to be the newest 2018 version, which was not available when we write the first version of the manuscript. The Planck 2018 lensing maps include a SZ cleaned lensing map, we use it in the revised manuscript to calculate \phi x y to prevent the influence of tSZ contamination in \phi map.

- Why not apply at least a Gaussian beam correction? It is trivial and would make the plots more immediately informative.

We want to make the plots to be apparently the same as Waerbeke et al, 2014.

- The method used to estimate error bars here is rather crude. It would be more robust to at least estimate them from the auto-spectra of the maps (the standard expression for this can be found in many papers). Even more robust would be to use simulations of the data sets, e.g., the Planck CMB lensing simulations.

Thanks for your suggestion. We adopt the auto-spectra to calculate the errorbar (see eq.13). This lowers the errorbars a little bit and thus affects the results a little bit.

Results:
- Fig. 5 indicates that the CIB leakage into the tSZ map is largest at low ell - do the authors have an explanation for this?

Because CIB x \phi is largest at low ell.

- Note that Hurier (2015) finds essentially an identical result for the CIB contamination to the tSZ - CMB lensing cross-correlation. This result should be cited and discussed: https://arxiv.org/abs/1701.09047
In addition, Hill & Spergel (2014) subtract a bias of this magnitude from the measured cross-correlation. This should also be mentioned explicitly.

We refer to Hurier(2015) in the revised manuscript.

Appendix A:
- The statements about the ILC method are not correct. In its original incarnation, the ILC method does not "project out" or "null" any contaminants. It simply minimizes the variance in the final ILC map, subject to the constraint of preserving the signal of interest. For example, if all of the input maps are noise-dominated, the ILC combination will essentially just inverse-noise-weight the maps in the linear combination (again, subject to the constraint of preserving the signal of interest), and thereby will not null any foreground.

Corrected.

- Eq. A10 should be $c_{\alpha i}$ on the LHS.

Corrected

- The calibration factors and unit conversions for the 545 GHz and 857 GHz channels are rather uncertain (5-10%). Are these uncertainties propagated into the final results, or investigated somehow?

We double check the table given in https://wiki.cosmos.esa.int/planckpla2015/index.php/UC_CC_Tables and find the uncertainty is 1% for 857GHz and 0.034% for 545GHz. 

- In the discussion around Eq. A14, I am confused as to the definition of the domain D. Is it the entire unmasked sky region? If so, this is not actually a true needlet ILC. The needlet ILC uses a spatially adaptive approach as well, where the domain D is local in real space, and its size is adapted for the needlet scale under consideration. If the entire unmasked sky is used, then the method becomes equivalent to a harmonic-space ILC, computed within a broad harmonic window corresponding to the needlet filter used. Additional comment: I now see that this is explicitly stated at the end of the second-to-last paragraph in A.2. I am extremely surprised that this naive method gives error bars consistent with those from the full NILC technique, as the residual Galactic foregrounds should be much larger in this map. The authors should include a comparison of the two maps similar to Fig. A2, but in a region closer to the Galactic plane.
- In Fig. A2, it would be useful to also include a panel showing the difference (y_Planck - y_Rec) between the two maps.

We include a comparison of the two maps as well as a difference map in a lower lat region. (see Fig.A2) There are some difference at large scales coming from galactic residual. As the region that we are probing is farther from the Milky Way than Planck’s y map, the galactic residual is lower so we argue that it is not crucial to use local domain D.

- "The reconstructed tSZ map is obtained by simply co-adding tSZ maps in all needlet windows." - this is not correct at face value - the final step before co-adding in the NILC procedure is to re-apply the needlet filter once more. Is this step applied? If not, the method is not unbiased, in the sense that the power in the input sky maps is not preserved.

We indeed did what you say here (re-apply the needlet filter again before co-adding). We’ve modified the text.

- "We smooth all the six CIB maps to an angular resolution of 10 arcmin and subtract them from the raw sky maps to make CIB-subtracted sky maps" - are the raw sky maps smoothed to the same resolution before the subtraction is performed?

Yes. Please check Section A.2 step 2.

- I am puzzled by the discussion at the beginning of A.4. I am not aware of any evidence from Planck (or elsewhere) for more than one or two Galactic dust components. More may be present at much fainter levels, but for describing the Planck data, one (or perhaps two) components suffices. Thus, why can these not be projected out?

Since T_d and beta_d both vary a cross the sky, it is not possible to formally describe the galactic dust to be a single component. To solve this issue, the Planck collaboration adopts a Generalized ILC (1605.09387) to disentangle the dust components. 
Our idea here is to choose one dust component (one set of {T_d, \beta_d}) to be projected out. When we vary \beta_d, the galactic dust residual in the y map changes. We want to test whether this residual influence the cross-correlations.

- "As in subsection A.3, CIB signal is subtracted out before producing the y map." - isn't this a somewhat risky step, since there is surely some Galactic dust in the CIB maps, and thus this subtraction will change the effective SED of the Galactic dust component, thereby rendering the nulling procedure ineffective?
The dust residual in CIB signal provides an additional change to the dust residual. This section is only a qualitative test so we can only check whether the dust residual changes the cross-correlation but we cannot quantify it at this stage.
